Dalorex: A Data-Local Program Execution and Architecture for Memory-bound Applications

Applications with low data reuse and frequent irregular memory accesses, such as graph or sparse linear algebra workloads, fail to scale well due to memory bottlenecks and poor core utilization. While prior work with prefetching, decoupling, or pipelining can mitigate memory latency and improve core utilization, memory bottlenecks persist due to limited off-chip bandwidth. Approaches doing processing in-memory (PIM) with Hybrid Memory Cube (HMC) overcome bandwidth limitations but fail to achieve high core utilization due to poor task scheduling and synchronization overheads. Moreover, the high memory-per-core ratio available with HMC limits strong scaling. We introduce Dalorex, a hardware-software co-design that achieves high parallelism and energy efficiency, demonstrating strong scaling with >16,000 cores when processing graph and sparse linear algebra workloads. Over the prior work in PIM, both using 256 cores, Dalorex improves performance and energy consumption by two orders of magnitude through (1) a tile-based distributed-memory architecture where each processing tile holds an equal amount of data, and all memory operations are local; (2) a task-based parallel programming model where tasks are executed by the processing unit that is co-located with the target data; (3) a network design optimized for irregular traffic, where all communication is one-way, and messages do not contain routing metadata; (4) novel traffic-aware task scheduling hardware that maintains high core utilization; and (5) a data placement strategy that improves work balance. This work proposes architectural and software innovations to provide the greatest scalability to date for running graph algorithms while still being programmable for other domains.

==> txt/TODOs.tex <==

1) From the Arch perspective:

From the literature in graph processing, PIM-based proposals are the direct comparison with Dalorex, since they also have a memory system that scales with the amount of computing resources, and they also use ISA-programmable cores that can execute applications outside the graph domain.
From these works we compare with Tesseract~\cite{tesseract}.
We also have simulated a more recent PIM-based approach GraphQ~\cite{2019graphq} which reported 3.3$\times$ performance and 1.8$\times$ energy improvements on average over Tesseract.
However, despite communicating with the authors, we were unable to obtain the cycle and energy values from simulation outputs that matched their results.
We do not include GraphQ in our discussion because the runtime and energy consumption we reproduced were 3.2$\times$ and 4.6$\times$ bigger (geomean), respectively, compared to these publications.

We also looked at the literature in graph accelerators, i.e., those with a specialized hardware pipeline to process the different stages of graph traversing, and focused on Polygraph---the latest work.
We evaluated the code that the authors kindly provided, and experimentally confirmed that Polygraph's performance plateaus after 16 cores, while \proj{} continues to scale.
This is expected since that configuration already saturates the 512GB/s of DRAM bandwidth.

When running \proj{} with equal number of processing elements, its performance is, in geomean, within

We observed that a configuration with an equal amount of processing elements, 256, we are within \% of their performance across the same datasets we evaluated in Fig.5.
However, when we try larger configurations, they don't scale because of having saturated the memory bandwidth. When looking at both approaches with 1024 processing elements, we find that \proj{} is X$\times$ more performant.

Polygraph is not designed for scalable, but hardware acceleration.
We compare with Tesseract because it's the memory scalable solution.
We wanted to confirm our expectation, and we experimentally found that Polygraph didn't scale performance after using 256 processing elements because of being limited by DRAM BW.
For a smaller configuration using 64 processing elements (4 Polygraph cores with 16-way parallelism), we found that the performance was within a 20\% range, in geomean.

Because Poly aims at optimizing load-balance between processing elements, once BW and network resources are not constraint, we cannot directly compare with them.

2) Software programmable. Scalability of the memory system.

3) How we win
They use heuristic, decide based on data-local.

-CONCLUSION: say about reproducing results, open source repo? or say Artifact evaluation
-Mention ISA programmable in Approach
-Dalorex-full on Figure 5
-Explain how the code is split? Talk about generalized compiler passes? Like Pipette or Desc, DEC++
-Talk about how eDRAM sucks in terms of density.
+Related work with SAM&TAM
+Related work wth Execution Migration Machine (EM) MIT, Devadas

==TEXT==
-Core to scratchpad area ratio?
-Refine claims
-mention strong scaling, as a way that we can do a graph partition with many more cores
-Better explain our 2MB sweet spot

-Refactor Mesh to matrix of tiles, interconnected as a torus or a mesh
-Replace Kron with RMAT??
-Replace 'Nodes' with 'Vertices', that's how they call them at Graphit



-Lower Effective bandwidth on DRAM with irregular Apps
-Embedded DRAM? 2-8MB mem per core. Limits of parallelization? the limit is more on the chip size. At wafer scale latency also affects.
Larger graphs just use more chips.
\textbf{Limitation}: Can't do a huge graph with a single chip. You could do that with HMC, but then we aren't parallelizing as much as we could.
If the point is to execute any size with a single chip, then eDRAM (out of the scope of this paper), if the point is to execute it fast, then we can parallelize more.










==FUTURE WORK, Outside the scope of this paper==

the only way to improve is by adding special instructions to the core for graph operations, what makes it slowly become an accelerator
And then the paper would be a network of small accelerators
Works have been proposed for doing ML-friendly thin core, manycores but not as much for graph-apps friendly

-cache-duality for different operating modes on manycores.
-chiplet integration vs monolitic chip, chiplets could contain a replica, to reduce inter chiplet communication
-Two types of SRAM memory or voltage scaling with ~\cite{variable_mem}, e.g. for Edge and Node arrays.
-In-depth comparison of DRAM and SRAM power with irregular accesses?

-Implementing global barrier?
-library of apps split into dalorex code.

==SIMULATOR==
-Nicer way to count instructions -> migrate to LLVM? 
In a similar fashion as MosaicSim simulates instructions.
-Integrate into MosaicSim


## HASHING
Hash the graph instead of the processing. Low bit hashing would involve extra Route3-1 communication. We don't want to have nodes separately, because of begin end redundancy
Not give extra explanation, just assume the graph is not sorted, re-hash
Not do:
Hashing type is select-able per task! task4 to task1, no hashing? then how to send the seed? the seed could also be in software, as a variable assigned to 1 of the tiles, value 0 (root) doesn't care about hashing
Pad nodes/edges to be multiple of #cores, so that the last tile also contains as many cores. Those nodes would have no neighbors
